VoiceMem: Streaming Dual-Brain Memory for Real-Time Interaction

Conversational systems, such as duplex speech language models (SLMs), still lack a streaming, accurate, and empathetic memory system as their soul. We introduce VoiceMem, a simple memory architecture with a parallel informational left brain, an emotional right brain, and streaming memory I/O mechanisms. We further build a complete pipeline for memory-aware SLM training, long-horizon evaluation, and decoupled deployment with interchangeable memory backends. Experiments and real-world deployment show three advantages: i) Accuracy: under top-5 retrieval, the left brain outperforms classical systems such as Mem0 at top-200 by nearly 30 points; ii) Emotional & Personal: the right brain, with short- and long-horizon affective attribution and dual-node persona modeling, achieves state-of-the-art performance across three persona benchmarks and improves the aggregate score by 4.29 points over the previous best system; and iii) Real-Time & Cheap: VoiceMem completes retrieval in 134 ms, well within standard VAD latency, adding no extra conversational delay while maintaining high accuracy and low cost. These results show that VoiceMem provides a practical memory foundation for real-time, personalized, and emotionally aware speech interaction.

==> experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  VoiceMem — Experiments (self-contained).
%%  main.tex 无需任何改动。所需宏包你的 main.tex 已全部加载：
%%  booktabs graphicx multirow caption tabularx xcolor[table] adjustbox
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
% -- 本节所需定义（已存在则跳过，不会冲突）--
\providecommand{\ph}[1]{\textcolor{red}{#1}}
\definecolor{headerblue}{RGB}{234,240,250}
\providecolor{srcblue}{RGB}{18,62,138}
\providecolor{estorange}{RGB}{201,110,17}
\providecommand{\src}[1]{\textcolor{srcblue}{#1}}
\providecommand{\est}[1]{\textcolor{estorange}{#1}}
\expandafter\ifx\csname NC@rewrite@C\endcsname\relax
  \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\fi
% -- 排版：图文间距 / 页面空洞 / 浮动体分布 --
\setlength{\textfloatsep}{8pt plus 2pt minus 2pt}
\setlength{\intextsep}{8pt plus 2pt minus 2pt}
\setlength{\floatsep}{8pt plus 2pt minus 2pt}
\setlength{\abovecaptionskip}{5pt}
\setlength{\belowcaptionskip}{2pt}
\renewcommand{\topfraction}{0.94}
\renewcommand{\bottomfraction}{0.65}
\renewcommand{\textfraction}{0.05}
\renewcommand{\floatpagefraction}{0.88}
\setcounter{topnumber}{4}
\setcounter{bottomnumber}{3}
\setcounter{totalnumber}{6}
%% no running head in this section: the rule and the section name cost two
%% text lines on every page. Move \pagestyle{plain} to the preamble to drop
%% them document-wide.
\pagestyle{plain}\thispagestyle{plain}
%% Tighter leading. article's default at 10pt is 12pt baselineskip; 0.94 puts it
%% near 11.3pt. Move this to the preamble to apply document-wide.
\linespread{0.94}\selectfont
%% Tighter headings. titlesec is not loaded by the class, so we redefine the
%% two levels through \@startsection directly (we are inside \makeatletter).
\renewcommand\section{\@startsection{section}{1}{\z@}%
  {-10pt \@plus -2pt \@minus -2pt}{4pt}{\normalfont\Large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
  {-7pt \@plus -1pt \@minus -2pt}{2.5pt}{\normalfont\large\bfseries}}
%% run-in \paragraph: the default 3.25ex before-skip leaves the three Settings
%% blocks floating apart from one another.
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
  {1.1ex \@plus .3ex \@minus .2ex}{-0.55em}{\normalfont\normalsize\bfseries}}
\raggedbottom
\setlength{\@fptop}{0pt}
\setlength{\@fpsep}{16pt}
\setlength{\@fpbot}{0pt plus 1fil}
\setlength{\@dblfptop}{0pt}
\setlength{\@dblfpsep}{16pt}
\setlength{\@dblfpbot}{0pt plus 1fil}
\makeatother
% -- 浮动栅栏：小节边界处强制排空队列，避免图表漂到后面几页 --
\providecommand{\floatbarrier}{\par\bigskip\penalty-200\relax
  \@ifundefined{FloatBarrier}{\clearpage}{\FloatBarrier}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!t]
\centering
% ==================== Table 1 ====================
\caption{\textbf{Factual memory results.} LLM-judge score (\%, $\uparrow$).
$\ddagger$: responses generated by our fine-tuned \ph{Qwen3.5-Omni} instead of
GPT-4o-mini.}
\label{tab:left}
\vspace{-0.1em}
{\fontsize{8.5pt}{10pt}\selectfont
\setlength{\tabcolsep}{2.59pt}
\renewcommand{\arraystretch}{0.92}
\begin{tabular}{@{}l *{11}{C{0.92cm}} C{0.92cm}@{}}
\toprule
\multirow{2}{*}{\textbf{Method}}
  & \multicolumn{4}{c}{\textbf{LoCoMo}}
  & \multicolumn{4}{c}{\textbf{LongMemEval}}
  & \multicolumn{3}{c}{\textbf{Memora}}
  & \multirow{2}{*}{\textbf{Avg.}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-12}
  & Single & Multi & Temp. & Open
  & Extr. & Multi & Upd. & Temp.
  & Rem. & Rec. & Rea. & \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Reference}}} \\
Full-Context
  & 75.87 & 72.27 & 70.29 & 57.45
  & 45.45 & 73.92 & 78.21 & 31.58
  & \textbf{85.54} & 52.10 & 22.67 & 60.49 \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Memory Engines}}} \\
Mem0
  & 67.13 & 51.15 & 55.51 & 72.93
  & 62.82 & 46.21 & 70.12 & 40.15
  & 40.42 & 52.58 & 16.00 & 52.27 \\
Zep
  & 66.91 & 53.70 & 60.29 & 43.82
  & 47.46 & 74.44 & 54.10 & 34.62
  & 33.36 &37.38  &3.50 & 46.33 \\
LangMem
  & 62.23 & 47.92 & 23.43 & 71.12
  & 55.13 & 20.30 & 66.67 & 15.79
  & 71.16 & 48.88 & 30.00 & 46.60 \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Agent Memory}}} \\
A-MEM$^{\dagger}$
  & 39.79 & 18.85 & 54.05 & 49.91
  & 84.62 & 48.87 & 64.11 & 47.36
  & 71.82 & 35.04 & 2.00 & 46.95 \\
MemoryOS
  & 30.00 & 80.00 & 48.72 & 64.29
  & 58.10 & 31.06 & 48.72 & 32.33
  & 15.24 & 38.86 & 1.50 & 40.80 \\
MemOS$^{\dagger}$
  & 81.09 & 67.49 & 75.18 & 55.90
  & 86.77 & 70.70 & 74.33 & 77.49
  & 51.84 & \textbf{62.64} & 20.66 & 65.83 \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Personal Memory}}} \\
MemoryBank$^{\dagger}$
  & 21.25 & 18.40 & 31.50 & 26.28
  & 23.33 & 26.00 & 14.00 & 20.00
  & 22.22 & 41.88 & 1.42 & 22.39 \\
EverMemOS$^{\dagger}$
  & 90.12 & 90.43 & 88.16 & 69.79
  & 85.71 & 73.68 & 89.74 & 77.44
  & 17.21 &33.27 &16.67  &66.57 \\
Emotional RAG
  & 19.62 &25.53 &34.89 &13.54
  &40.00 &55.00 &70.00 &65.00
  & 51.16 & 39.38 & 14.75 & 38.99 \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Ours}}} \\
\textbf{VoiceMem}
  & \textbf{90.60} & \textbf{86.60} & \textbf{85.8} & \textbf{79.60}
  & \textbf{80.00} & 75.00 & \textbf{77.50} & \textbf{95.00}
  & 66.80 &50.50 &30.70
 & \textbf{74.69} \\
\bottomrule
\end{tabular}
}
% ==================== Space between tables ====================
\vspace{-0.3em}
% ==================== Table 2 ====================
\caption{\textbf{Persona memory results.} LLM-judge score (\%, $\uparrow$).}
\label{tab:right}
\vspace{-0.1em}
{\fontsize{8.5pt}{10pt}\selectfont
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.92}
\begin{tabular}{@{}l *{11}{C{0.95cm}} C{0.95cm}@{}}
\toprule
\multirow{2}{*}{\textbf{Method}}
  & \multicolumn{4}{c}{\textbf{ES-MemEval}}
  & \multicolumn{5}{c}{\textbf{PersonaMem}}
  & \multicolumn{2}{c}{\textbf{PersonaLens}}
  & \multirow{2}{*}{\textbf{Avg.}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-10}\cmidrule(lr){11-12}
  & IE & TR & CD & UM
  & Rec. & Gen. & Evol. & Reason & Reco.
  & Per. & TCR & \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Reference}}} \\
Full-Context
  & 20.20 & 19.60 & 12.10 & 21.70
  & 41.00 & 46.00 & \textbf{68.00} & 77.00 & 37.00
  & 75.00 & 91.08 & 46.24 \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Memory Engines}}} \\
Mem0
  & 75.10 & 56.70 &72.30 & 64.20
  & 32.13 & 57.89 & 54.68 & 80.81 & 52.73
  & 82.25 & 92.39 & 65.56 \\
Zep
  & 66.80 & 42.30 & 64.20 & 58.00
  & 35.30 & 42.10 & 34.50 & 50.50 & 36.40
  & 58.50 & 82.74 & 51.94 \\
LangMem
  & 18.80 & 15.00 & 20.40 & 22.70
  & 31.29 & 8.77 & 53.24 & 81.82 & 40.00
  & 77.45 & 92.99 & 42.04 \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Agent Memory}}} \\
A-MEM$^{\dagger}$
  & 67.80 & 58.30 & 67.00 & 56.70
  & 63.01 & 57.89 & 54.68 & 85.86 & 69.09
  & 62.50 & 83.26 & 66.01 \\
MemoryOS
  & 43.90 & 30.50 & 41.00 & 41.50
  & 47.06 & 56.14 & 32.37 & 48.48 & 47.27
  & 55.75 & 82.01 & 47.82 \\
MemOS$^{\dagger}$
  &77.70 &64.60 & 66.30 & 73.50
  & 72.72 & 56.14 & 58.27 & 78.79 & \textbf{72.72}
  & 82.75 & 93.47 & 72.45 \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Personal Memory}}} \\
MemoryBank$^{\dagger}$
  & 43.00 & 35.20 & 42.70 & 38.70
  & 35.29 & 49.12 & 51.08 & 56.57 & 40.00
  & 64.50 & 80.66 & 48.80 \\
EverMemOS$^{\dagger}$
  & 66.80 & 50.70 & 59.60 & 45.90
  & 47.06 & 47.37 & 41.01 & 43.43 & 56.36
  & 63.25 & 79.91 & 54.67 \\
Emotional RAG
  &82.30 & 67.10 &\textbf{77.30} & 73.70
  & 52.94 & 61.40 & 44.60 & 58.59 & 43.64
  & 64.25 & 82.00 & 64.77 \\
\midrule
\multicolumn{13}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Ours}}} \\
gpt-4o-mini
  &\textbf{82.80} &\textbf{67.30} & 69.10 &\textbf{74.00}
  & \textbf{76.47} & \textbf{64.91} & 51.08 & \textbf{83.84} & 70.91
  & \textbf{83.75} & \textbf{94.63} & \textbf{72.94} \\
self-trained$^{\ddagger}$
  &81.20 &64.70 &73.50 &71.90
  & \ph{--} & \ph{--} & \ph{--} & \ph{--} & \ph{--}
  & \ph{--} & \ph{--} & \ph{--} \\
\bottomrule
\end{tabular}
}
\end{table}

\section{Experiments}
\label{sec:experiments}

In this section, we conduct a series of experiments to answer four questions:

\begin{tcolorbox}[
colback=gray!8,
colframe=black,
boxrule=0.6pt,
arc=3mm,
left=2mm,
right=2mm,
top=1.5mm,
bottom=1.5mm
]
\textbf{(RQ1) Does VoiceMem preserve accuracy on both information and persona?}
\emph{\S\ref{sec:main}}
\vspace{1mm}

\textbf{(RQ2) Does VoiceMem hold up under complex, very long multi-turn audio input?}
\emph{\S\ref{sec:voice}}
\vspace{1mm}

\textbf{(RQ3) Do the left- and right-brain update adapt to long-horizon use, and why?}
\emph{\S\ref{sec:abl}}
\vspace{1mm}

\textbf{(RQ4) Does the architecture transfer across different underlying memory systems?}
\emph{\S\ref{sec:abl}}
\end{tcolorbox}

%% ==================================================================
\subsection{Settings}
\label{sec:settings}

\paragraph{Benchmarks.}
We evaluate on three families.
\emph{(i) Information memory}: LoCoMo~\citep{locomo},
LongMemEval (S)~\citep{longmemeval}, and Memora~\citep{memora}.
\emph{(ii) Persona memory}: ES-MemEval~\citep{esmemeval},
PersonaMem~\citep{personamem}, and PersonaLens~\citep{personalens}.
\emph{(iii) Voice-grounded memory}: ChatMem-Bench, with $347$ questions
over $47.86$ hours of audio in four ability groups and fourteen sub-categories.

\paragraph{Baselines.}
Ten systems in four groups.
\emph{(i) Reference}: Full-Context.
\emph{(ii) Memory engines}: Mem0~\citep{mem0}, Zep~\citep{zep},
LangMem~\citep{langmem}.
\emph{(iii) Agent memory}: A-MEM~\citep{a-mem}, MemoryOS~\citep{memoryos},
MemOS~\citep{memos}.
\emph{(iv) Personal memory}: MemoryBank~\citep{memorybank},
EverMemOS~\citep{evermemos}, Emotional RAG~\citep{emotionalrag}.

\paragraph{Implementation details.}
All baseline systems use GPT-4o-mini~\citep{gpt4omini} as the backbone LLM and
text-embedding-3-small~\citep{textembedding3small} as the embedding model, with
temperature $0$. VoiceMem is evaluated under six retrieval settings,
$K\in{3,10,100}$. Detailed implementations and system-specific configurations
are provided in the appendix.

%% ==================================================================
\subsection{Main Results}
\label{sec:main}

\textbf{For [RQ1]}, \textsc{VoiceMem} retrieves dense memory on both information and persona. As presented in Tab.~\ref{tab:left}, our method leads on 9 of 11 sub-categories across all baselines. It averages 74.03, beating Mem0, its own storage backend, by +21.8 and full-context processing, which sees the entire history, by +13.3. The margin is widest when several memories must arrive together (e.g., temporal reasoning, +54.9) and narrowest on open-domain questions, which one good memory already answers. As presented in Tab.~\ref{tab:right}, our method reaches 73.28 on twelve persona sub-categories and passes the strongest baseline, MemOS, by +0.9. The reference inverts on ES-MemEval, where full context scores 12.10 on conflict detection and 21.70 on user modeling, against 67.79 and 70.10 for ours, i.e., the evidence sits in its input and it still cannot attribute it. Notably, both tables are produced at a retrieval budget an order of magnitude below the top-100 setting conventional in text-agent memory, which indicates that the gains come from a denser candidate pool rather than a larger one.

%% ==================================================================
\subsection{ChatMem-Bench: Long-Horizon Audio Assistant Memory}
\label{sec:voice}

\begin{table}[!t]
\centering
\caption{\textbf{ChatMem-Bench results.} LLM-judge score (\%, $\uparrow$).}
\label{tab:voice}
\vspace{-0.1em}
{\fontsize{7.8pt}{10pt}\selectfont
\setlength{\tabcolsep}{0.22pt}
\renewcommand{\arraystretch}{0.85}
\begin{tabular}{@{}l *{14}{C{0.88cm}} C{0.88cm}@{}}
\toprule
\multirow{2}{*}{\textbf{Method}}
  & \multicolumn{4}{c}{\textbf{Information}}
  & \multicolumn{3}{c}{\textbf{Persona}}
  & \multicolumn{3}{c}{\textbf{Affective Attr.}}
  & \multicolumn{4}{c}{\textbf{Paraling.\&Env.}}
  & \multirow{2}{*}{\textbf{Avg.}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-15}
  & Upd. & Temp. & Synt. & Abst.
  & Prof. & Pref. & Impl.
  & Attr. & Agd. & Phras.
  & Bsr. & Asi. & Mul. & Asa. & \\
\midrule
\multicolumn{16}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Reference}}} \\
Full-Context
  & 62.07 & 42.11 & 68.42 & 57.89 & 61.11 & 65.22 & 41.17
  & 50.00 & 57.14 & 37.78 & 11.76 & 22.58 & 26.92 & 90.00 & 50.18 \\
\midrule
\multicolumn{16}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Memory Engines}}} \\
Mem0
  & 55.17 & 31.57 & 84.21 & 68.42 & 66.67 & 78.26 & 52.94
  & 16.67 & 61.90 & 46.67 & 11.76 & 3.23 & 11.54 & 93.00 & 52.88 \\
Zep
  & 37.93 & 15.78 & 63.16 & 63.16 & 50.00 & 69.57 & 35.29
  & 8.33 & 57.14 & 33.33 & 5.88 & 9.68 & 7.69 & 91.50 & 42.15 \\
LangMem
  & 58.62 & 21.05 & 73.68 & 78.95 & 61.11 & 73.91 & 47.05
  & 41.67 & 47.62 & 42.22 & 11.76 & 12.90 & 15.38 & 93.00 & 49.68 \\
\midrule
\multicolumn{16}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Agent Memory}}} \\
A-MEM
  & 41.38 & 10.53 & 68.42 & 73.68 & 38.89 & 73.91 & 41.17
  & 25.00 & 52.38 & 44.44 & 23.53 & 9.68 & 3.85 & 93.65 & 44.08 \\
MemoryOS
  & 51.71 & 36.84 & \textbf{89.47} & 73.68 & 44.44 & 82.61 & 35.29
  & 25.00 & 52.38 & 35.55 & 5.88 & 19.35 & 15.38 & 95.59 & 50.35 \\
MemOS
  & 72.41 & 31.57 & 52.63 & 84.21 & \textbf{77.78} & 78.26 & 47.05
  & 50.00 & 71.43 & 46.67 & 17.65 & 12.90 & 19.23 & 93.46 & 55.14 \\
\midrule
\multicolumn{16}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Personal Memory}}} \\
MemoryBank
  & 41.38 & 5.26 & 47.37 & 63.16 & 38.89 & 52.17 & 29.41
  & 8.33 & 42.86 & 24.44 & 23.53 & 6.45 & 7.69 & 94.49 & 38.84 \\
EverMemOS
  & 44.83 & 26.32 & 63.16 & \textbf{94.74} & 50.00 & 69.57 & 52.94
  & 33.33 & 66.67 & 37.78 & 11.76 & 9.68 & 23.08 & 94.41 & 52.02 \\
EmotionalRAG
  & 34.48 & 10.53 & 57.89 & 73.68 & 44.44 & 60.87 & 58.82
  &  58.33 & 42.22 & 11.76 & 3.23 & 3.85 & 94.55 & 42.76 \\
\midrule
\multicolumn{16}{@{}l}{\cellcolor{headerblue}\textit{\textbf{Ours}}} \\
\textbf{VoiceMem}
  & \textbf{79.31} & \textbf{47.37} & 73.68 & 89.47 & 72.22 & \textbf{86.96} & \textbf{64.71}
  & \textbf{66.67} & \textbf{76.19} & \textbf{51.11} & \textbf{47.06} & \textbf{45.16}
  & \textbf{52.84} & \textbf{98.50} &\textbf{ 68.27} \\
\textbf{VoiceMem}$^{\ddagger}$
  & \ph{--} & \ph{--} & \ph{--} & \ph{--} & \ph{--} & \ph{--} & \ph{--}
  & \ph{--} & \ph{--} & \ph{--} & \ph{--} & \ph{--} & \ph{--} & \ph{--} & \ph{--} \\
\bottomrule
\end{tabular}
}
\end{table}

As briefly introduced in Sec.~\ref{sec:chatmem-bench-method}, \underline{\textbf{\textsc{ChatMem-Bench} evaluates whether a memory system can}}  \underline{\textbf{consolidate long-term speech interaction, across complex environments, affect, and informat-}}  \underline{\textbf{ion into a good voice assistant}}. It contains \textbf{500} questions drawn from \textbf{15,314} turns and 67.86 hours of dialogue, and every session is \textbf{\textit{curated by humans}}, from choosing the topic to constructing the memory world and designing the challenge. As shown in Tab.~3, the benchmark has four dimensions with 14 fine-grained categories. From left to right, Information covers \textit{update tracking}, \textit{temporal reasoning}, \textit{synthesis}, and \textit{abstention}; Persona covers \textit{profile constraints}, \textit{preference-aligned recommendation}, and \textit{implicit-need inference}; Affective Attribution covers \textit{emotion--target attribution}, \textit{attachment-guided decisions}, and \textit{affect-aware phrasing}; Paralinguistics \& Environment covers \textit{background-sound recall}, \textit{acoustic-scene inference}, \textit{multi-user conversational memory}, and \textit{acoustic style adaptation}.

\textbf{For [RQ2],} as shown in Tab.~\ref{tab:voice}, \textsc{VoiceMem} leads on 13 of the 14 categories, and the gap is widest on Paralinguistics \& Environment, where a transcript carries no evidence at all: every text system lands between 3.23 and 26.92 on the three acoustic categories, while ours reaches 47.06 to 52.84. Affective Attribution shows the opposite, i.e., text baselines stay competitive because word choice already carries most of the affective signal, and the audio increment appears instead on attachment-guided decisions and affect-aware phrasing. Notably, this accuracy costs 383 tokens and 1,459 ms, an order of magnitude below Mem0 and faster than every baseline.

%% 原 fig1_streaming.pdf（二维 deployment frontier）已删除：
%% 它和 §5.4 的三维前沿图讲的是同一件事，两张 caption 都是 "deployment frontier
%% on LoCoMo"，重复。附录 appendix_deployment.tex 里 "the full per-system table
%% behind Figure~\ref{fig:stream}" 这句现在会悬空，需要改成指向 §5.4 的
%% Figure~\ref{fig:frontier3d}。

%% %% %% ==================================================================
%%  VoiceMem — §5.4 Ablation and Analysis → §5.5 Case Study → Appendix
%%  一跳邻居表（原 Table 4）和涌现表（原 Table 5）已移到附录 App.~\ref{app:abl}。
%%
%%  需要的图（放 visuals/，覆盖同名旧文件）：
%%    visuals/vm_combined.png   —— 左 3D 前沿 + 右 K-sweep，一张图两个 caption
%%    fig3_dualbrain.png        —— 双脑散点（第 2 页顶 teaser）
%%    fig4_component.png        —— 四数据集组件消融柱状图
%%
%%  依赖：booktabs graphicx multirow caption adjustbox xcolor + \ph{} \est{} C{}
%%  注意：文件末尾的 \appendix 如果 main.tex 里已经有，删掉这一行。
%% ==================================================================
\subsection{Ablation and Analysis}
\label{sec:abl}

%% 本节内每页顶部只允许一个浮动体。前面的排版块把 topnumber 设成了 4，
%% 那样双脑散点会跟着上面那组图一起挤进同一页的页顶，而不是落到下一页顶。
%% 节末会恢复原值。
\setcounter{topnumber}{1}
\setcounter{totalnumber}{2}

%% ---------- 第 1 页顶：合成图（3D + 折线）+ 组件消融柱状图 ----------
\begin{figure}[!t]
\centering
\includegraphics[width=0.97\linewidth]{visuals/vm_combined.png}
\vspace{-2mm}

\begin{minipage}[t]{0.42\textwidth}
\vspace{-3mm}
\captionof{figure}{\textbf{Time--cost--accuracy on LoCoMo.}}
\label{fig:frontier3d}
\end{minipage}
\hfill
\begin{minipage}[t]{0.55\textwidth}
\vspace{-3mm}
\captionof{figure}{\textbf{Retrieval-budget sweep on LoCoMo,}}
\label{fig:ksweep}
\end{minipage}
\end{figure}

\begin{figure}[t]
\centering
\vspace{-5mm}
\includegraphics[width=\linewidth]{fig4_component.png}
\captionof{figure}{\textbf{Component ablation at $K{=}5$,} one mechanism disabled
per bar. Each panel uses its own $y$-range; none starts at zero.}
\label{fig:component}
\end{figure}

\noindent
\textbf{[RQ1] Cost, accuracy and latency, together.}\quad
Figure~\ref{fig:frontier3d} plots all three axes at once. VoiceMem at $K{=}5$
reaches $91.2$ with $430$ memory tokens and $454$\,ms of retrieval. The strongest
baseline, EverMemOS, reaches $90.1$ with $1{,}899$ tokens: \textbf{$+1.1$ points
at $4.4\times$ fewer tokens.} Accuracy is flat past $K{=}5$ --- $K{=}10$ adds
$0.2$ points for $40\%$ more tokens, $K{=}100$ adds $0.9$ for $8\times$ --- and
latency does not grow with $K$, because schema routing keeps the candidate pool
small regardless of how many items are finally returned.

%% ---------- 第 2 页顶：双脑散点 teaser ----------
\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{fig3_dualbrain.png}
\caption{\textbf{What the two stores hold.} \emph{Left:} left-brain items by
semantic slot, with the two emergent sub-slots circled. \emph{Middle:} right-brain
items by module. \emph{Right:} right-to-left linking, ribbon width proportional to
link count.}
\label{fig:dualbrain}
\end{figure}

\noindent
\textbf{[RQ1] The two stores hold different things.}\quad
Figure~\ref{fig:dualbrain} reports structure rather than scores. The left store
holds $510$ items across six preset slots. Two further slots were never preset;
they emerged from the semantic graph and cover $254$ items, $43\%$ of the store.
Neither sits inside a single preset slot: \emph{Pets \& Outdoor} ($218$ items)
draws $48\%$ from \texttt{daily\_life}, $27\%$ from \texttt{health} and $17\%$
from \texttt{relationships}, and \emph{Engineering Project} ($36$ items) splits
between \texttt{work} ($39\%$) and \texttt{goals} ($31\%$). Both span all six
preset slots, so \textbf{emergence re-partitions the store across preset
boundaries rather than refining within them.} The right store holds $251$ items
in four modules, linked to left-brain slots by $280$ edges spread unevenly:
\texttt{daily\_life} receives $91$, \texttt{knowledge} $9$.

\vspace{0.3em}

\noindent
\textbf{[RQ3] Schema routing lowers the budget, not the ceiling.}\quad
Figure~\ref{fig:ksweep} sweeps $K$ on LoCoMo. \textbf{VoiceMem is highest at every
$K$, and the margin is widest where the budget is tightest:} $+13.3$ over Mem0 and
$+32.0$ over Emotional RAG at $K{=}1$, and $+4.1$ over EverMemOS at $K{=}5$. The
baselines need roughly $20\times$ the budget to catch up --- Zep reaches $90.2$
and Emotional RAG $87.8$ only at $K{=}100$, a level VoiceMem passes at $K{=}3$
with $362$ tokens. Removing schema routing separates the two VoiceMem curves at
small $K$ and they then converge: routing is worth $6.4$ points at $K{=}3$,
$0.05$ at $K{=}5$ and $K{=}10$, and the two stay within about $1$ point of each
other from $K{=}30$ to $K{=}100$. \textbf{Routing does not raise the ceiling; it
lowers the budget needed to reach it} --- with routing $430$ tokens suffice,
without it the same accuracy takes $K{=}30$ and $1{,}277$ tokens, $3\times$ the
cost.

\noindent
\textbf{[RQ3] Every mechanism contributes on every dataset.}\quad
Figure~\ref{fig:component} disables one mechanism at a time on four datasets.
All five ablations lose accuracy on all four. Schema routing is the largest loss
everywhere ($-9.9$ / $-5.3$ / $-6.7$ / $-4.4$ on LoCoMo / ES-MemEval /
ChatMem-Bench / Memora). The right brain
is next ($-6.3$ / $-4.3$ / $-5.4$ / $-4.4$), so \textbf{affect and persona carry
information the factual store does not.} Emergent clustering ($-5.5$ / $-2.0$ /
$-3.4$ / $-0.2$) and dual-horizon updating ($-5.4$ / $-2.0$ / $-3.2$ / $-1.4$)
are largest on LoCoMo, whose sessions are the longest, and smallest on Memora.
Joint retrieval is the smallest on two of four datasets ($-2.6$ / $-3.1$ / $-2.7$ / $-0.4$):
taking the union of two separately ranked lists is a workable fallback. Two
further ablations --- how a one-hop neighbour schema should enter the prompt, and
how cluster maintenance pays off as history grows --- are in
Appendix~\ref{app:abl}.

\vspace{0.3em}

\noindent
\begin{minipage}[c]{0.475\textwidth}
\textbf{[RQ4] The index transfers across backends.}\quad
The index assumes three things of the store beneath it: items addressable by
identifier, a similarity primitive, and write semantics that can \textsc{update}
rather than only append. Table~\ref{tab:backend} mounts it on three stores with no
threshold retuned. \textbf{All three improve, by $15.8$ to $28.7$ points}, so the
gain is not specific to one store. Two caveats: Mem0 is our default backend, so
that row \emph{is} the full system; and Zep and Mem0 start within $0.1$ points of
each other yet end $14.7$ apart, so the store still bounds how much the index can
recover.
\end{minipage}
\hfill
\begin{minipage}[c]{0.485\textwidth}
\centering
\captionof{table}{\textbf{Backend transfer on LoCoMo,} without retuning.}
\label{tab:backend}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.04}
\begin{tabular}{@{}l C{1.15cm} C{1.15cm} C{1.15cm}@{}}
\toprule
\textbf{Backend} & \textbf{bare} & \textbf{+ ours} & $\Delta$ \\
\midrule
Mem0$^{\dagger}$ & 61.68 & \textbf{90.40} & \textbf{+28.72} \\
LangMem          & 77.00 & \textbf{92.76} & +15.76 \\
Zep              & 52.74 & \textbf{75.66} & +22.92 \\
\midrule
\textit{mean}    & 60.26 & \textit{86.27} & \textit{+22.47} \\
\bottomrule
\end{tabular}

\vspace{0.2em}
{\scriptsize $^{\dagger}$ Default backend; this row is the full system.}
\end{minipage}

%% 恢复本节开头临时改掉的浮动体上限
\setcounter{topnumber}{4}
\setcounter{totalnumber}{6}


